TACO: Taming Diffusion for in-the-wild Video Amodal Completion

Humans can infer complete shapes and appearances of objects from limited visual cues, relying on extensive prior knowledge of the physical world. However, completing partially observable objects while ensuring consistency across video frames remains challenging for existing models, especially for unstructured, in-the-wild videos. This paper tackles the task of Video Amodal Completion (VAC), which aims to generate the complete object consistently throughout the video given a visual prompt specifying the object of interest. Leveraging the rich, consistent manifolds learned by pre-trained video diffusion models, we propose a conditional diffusion model, TACO, that repurposes these manifolds for VAC. To enable its effective and robust generalization to challenging in-the-wild scenarios, we curate a large-scale synthetic dataset with multiple difficulty levels by systematically imposing occlusions onto un-occluded videos. Building on this, we devise a progressive fine-tuning paradigm that starts with simpler recovery tasks and gradually advances to more complex ones. We demonstrate TACO's versatility on a wide range of in-the-wild videos from Internet, as well as on diverse, unseen datasets commonly used in autonomous driving, robotic manipulation, and scene understanding. Moreover, we show that TACO can be effectively applied to various downstream tasks like object reconstruction and pose estimation, highlighting its potential to facilitate physical world understanding and reasoning. Our project page is available at https://jason-aplp.github.io/TACO.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

It is common to observe only partial and incomplete objects in video clips, as mutual occlusions are prevalent in the real world. Leveraging prior knowledge acquired over time, humans can infer complete object attributes, including shape, appearance, and motion, even from partial observations. However, recovering these attributes consistently in a video is highly ill-posed due to the inherent ambiguities in unobserved areas. Moreover, it remains unexplored how to effectively ``teach'' a model to develop this ``see-through'' capability. Nonetheless, such consistent and complete object-centric representations are crucial for understanding the physical world and enabling efficient abstract reasoning~\cite{locatello2020object}, facilitating numerous downstream tasks in areas like reconstruction, robotic manipulation, autonomous driving, and beyond.
% Partial observations of an instance are common in video clips due to mutual occlusion or being out of the camera’s field of view. While human beings can hallucinate spatially and temporally consistent underlying object attributes, including geometry, appearance, and motion for video understanding, this task is highly challenging and ill-posed due to the ambiguities in unobserved areas. Nevertheless, recovering complete object geometry, appearance, and motion given partially visible observations is crucial for many downstream applications, ranging from gaming and filmmaking to AR/VR and robotics.

Therefore, in this paper, we aim to tackle the problem of \textit{video amodal completion} (VAC) — recovering temporal-spatial consistent and complete object attributes given a monocular video with mutual occlusions, and we start by analyzing essential capabilities for accomplishing this task. The model must first comprehend how the camera and the object move over time within the video, then aggregate all the visible parts across different frames, and finally synthesize the hidden parts consistently and plausibly without altering the already observable ones. Indeed, this task can be decomposed into individual frames, where frame-wise amodal completion techniques~\cite{ozguroglu2024pix2gestalt, xu2024amodal, zhan2024amodal} can be applied. However, this paradigm lacks temporal and spatial awareness, making it hard to effectively aggregate all the visible partial observations and synthesize consistent underlying object attributes. Another line of research work opts to solve this problem as video inpainting~\cite{gao2020flow, ke2021occlusion, kim2019deep, lee2019copy, li2022towards, zeng2020learning}, which aims at filling in plausible content in masked areas. Despite the harmonious results with the video context, they lack the awareness of amodal objects within, leading to artifacts when inpainting unobserved parts of an object~\cite{li2024ag2manip}.


% However, this task is naturally ill-posed as there exists numerous possibilities in unobserved areas. Indeed, this problem can be decomposed to each frame and apply a frame-wise image amodal completion model~\cite{ozguroglu2024pix2gestalt, ehsani2018segan, zhan2020self} or amodal segmentation~\cite{ke2021deep, ling2020variational, qi2019amodal, reddy2022walt} and inpainting model~\cite{lugmayr2022repaint, xie2023smartbrush, corneanu2024latentpaint}. This kind of approach gives up the temporal and spatial consistency in the video, making it hard to naively guarantee frame-wise consistency due to the under-constraint setting. Another line of research work~\cite{gao2020flow, ke2021occlusion, kim2019deep, lee2019copy, li2022towards, zeng2020learning} focus on the task of video inpainting, which aims at restoring plausible and natural content in missing/occluded region. Despite the compelling harmonious results with the environment, few of them possess the awareness of objects within, leading to obvious artifacts when large occluded object regions are inpainted. Therefore, in this paper we not only focus on learning the occluded background area but every occluded object instance as well given a video clip.  %video inpainting & pix2gestalt, image inpainting, amodal segmentation & NVS tasks


==> sec/2_related.tex <==
\section{Related Work}
\label{sec:relwork}

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}




%-------------------------------------------------------------------------
\subsection{Type style and fonts}


%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_method.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
